Level lines of the Gaussian Free Field with general boundary data

We study the level lines of a Gaussian free field in a planar domain with general boundary data $F$. We show that the level lines exist as continuous curves under the assumption that $F$ is regulated (i.e., admits left and right limits at every point), and satisfies certain inequalities. Moreover, these level lines are a.s. determined by the field. This allows us to define and study a generalization of the SLE$_4(\underline{\rho})$ process, now with a continuum of force points. A crucial ingredient is a monotonicity property in terms of the boundary data which strengthens a result of Miller and Sheffield and is also of independent interest.

==> tex/gff_levellines_existence.tex <==
In this section we will show existence of the coupling described by Theorem \ref{thm::gff_levelline_coupling}. Recall we would like to prove that for $F$ on $\R$ which is regulated, so can be approximated uniformly by piecewise constant functions changing value only finitely many times, and which satisfies Condition (\ref{eqn::inequalities}),
there exists a coupling of a Loewner chain $K$ with a zero boundary  GFF $h$, such that $K$ is a level line of $h+F$. Moreover, we will show that $K$ is almost surely generated by a continuous and transient curve $\gamma$. 
 
To do this we will take a sequence of piecewise constant functions $F_n$ (changing value only finitely many times), which uniformly approximate $F$, and consider the level lines, denoted by $\gamma^{(n)}$, of $h+F_n$ for a zero boundary GFF $h$. Observe that we can choose the $F_n$ so that the level lines are a family of $\SLE_4(\underline{\rho}^L;\underline{\rho}^R)$ processes satisfying the conditions of Corollary \ref{cor::tightness}. Thus, the tightness given by the corollary will allow us to extract a subsequential limit. 


\begin{proposition}
\label{propn::weaklimit}
Let $F$ satisfy the conditions of Theorem \ref{thm::gff_levelline_coupling}. Suppose that $(F_n)_{n\in \N}$ are piecewise constant functions on $\R$, changing value only finitely many times. Let $h$ be a zero boundary  $\GFF$ and $\gamma^{(n)}$ be the level line of $h+F_n$ for each $n$. Suppose further that they are all parameterized by half plane capacity and that $(W^{(n)})_{n\in \N}$ are the corresponding family of driving functions.

Then, if the $(F_n)$ converge uniformly to $F$ on $\R$, we have that: 
\begin{enumerate}
\item [(1)] There exists a subsequence of the $\gamma^{(n)}$ which converges weakly in the space of continuous functions on $[0,\infty)$ with the topology of uniform convergence on compact subsets of $[0,\infty)$. 
\item [(2)] The limiting law describes a continuous curve from $0$ to $\infty$ in $\HH$ which generates a Loewner chain with a.s. continuous driving function.
\item [(3)] The limiting curve can be coupled with a zero boundary $\GFF$ $h$, as a level line of $h+F$.  
\end{enumerate}

\end{proposition}

\begin{remark} We will later see that this limiting law does not depend on the choice of approximation, as any continuous curve which can be coupled with a zero boundary $\GFF$ as a level line of $h+F$ must have a unique law: see Remark \ref{rmk::lawunique}. In particular, this tells us that we actually have convergence of the whole sequence in distribution.  \end{remark}

\begin{proof}[Proof of Theorem \ref{thm::gff_levelline_coupling}]
Theorem \ref{thm::gff_levelline_coupling} is a direct consequence of Proposition \ref{propn::weaklimit}.
\end{proof}
\begin{proof}[Proof of Proposition \ref{propn::weaklimit}, Items (1), (2)]
Note that the weak convergence directly follows from Corollary \ref{cor::tightness}, as does the fact that the limiting law corresponds to a continuous curve generating a Loewner chain with almost surely continuous driving function. 
\end{proof}
To prove Proposition \ref{propn::weaklimit}, Item (3), i.e. to see that the limiting curve can be coupled as a level line in the way we want, we will use Lemma \ref{lem::coupling_iff_martingale}. This tells us that if we define $\eta_t$ as in Definition \ref{def::gff_levelline} for the function $F$ and our limiting Loewner chain, we need only show that for each $z\in \HH$, the process $\eta_t(z)$ is a Brownian motion when reparameterized by minus the log conformal radius of $\HH\setminus K_t$ seen from $z$. {\color{blue} Change to the new version of Lemma 2.15.}


\begin{definition}
\label{defn::etatilde}
Suppose that $F$ is $L^1$ with respect to harmonic measure on $\R$ and that $\gamma$ is a continuous curve with continuous Loewner driving function. We set $\eta_t^0$ in the same way as in Definition \ref{def::gff_levelline}. 
Then for any $z\in \HH$ we can define, for $t$ less than the first time that $\gamma$ swallows $z$,
\[\eta_t(F, \gamma, z)=\eta_t^0(f_t(z))\]
as in Definition (\ref{def::gff_levelline}), emphasising the dependence on $F$ and $\gamma$. 
Finally, we let 
\[C_t(\gamma, z)=-\log \CR(z,\HH\setminus K_t)\] be minus the log conformal radius of $\HH\setminus K_t$ seen from $z$, and 
\[\tilde{\eta}_t(F, \gamma ,z)=\eta_{\tau(t)}(F, \gamma, z), \] 
where $\tau(t):= \inf\{s\geq 0: C_s(\gamma, z)=t\}$. 
\end{definition}

\begin{lemma}\label{lem::tildeeta_cvg_gamma}
Let $(\gamma^{(n_k)})$ be a subsequence of the random curves in Proposition \ref{propn::weaklimit}, parameterised by half plane capacity, which converge weakly to some $\gamma$ in the space of continuous functions on $[0,\infty)$ with the topology of uniform convergence on compacts. Then for every $z\in \HH$, \[\left(\tilde{\eta}_t(F, \gamma^{(n_k)},z)\right)_{t\geq 0} \xrightarrow{d}\left(\tilde{\eta}_t(F, \gamma,z)\right)_{t\geq 0}\]
in the space of continuous real-valued functions on $[0,\infty)$.
\end{lemma}

\begin{lemma}
\label{lemma::etaconvergence}
Let $(\gamma^{(n_k)})$ be a subsequence of the random curves in Proposition \ref{propn::weaklimit}, parameterised by half plane capacity, which converge weakly to some $\gamma$ in the space of continuous functions on $[0,\infty)$ with the topology of uniform convergence on compacts. Then for every $z\in \HH$, \[\left(\tilde{\eta}_t(F_{n_k}, \gamma^{(n_k)},z)\right)_{t\geq 0} \xrightarrow{d}\left(\tilde{\eta}_t(F, \gamma,z)\right)_{t\geq 0}\]
in the space of continuous real-valued functions on $[0,\infty)$.
\end{lemma}

\begin{proof}
By Lemma \ref{lem::tildeeta_cvg_gamma}, we have that \begin{equation}
\label{eqn::weakconvergence1}
(\tilde{\eta}_t(F, \gamma^{(n_k)},z))_{t\geq 0} \xrightarrow{d} \left(\tilde{\eta}_t(F, \gamma,z)\right)_{t\geq 0} 
\end{equation} with respect to the topology of uniform convergence on compacts. It is also clear that, for all $t,z$ and any curve $\gamma'$
\[\left|\tilde{\eta}_t(F_{n_k}, \gamma',z)-\tilde{\eta}_t(F, \gamma',z)\right| \leq \sup_{x\in \R}|F(x)-F_{n_k}(x)|.\] Indeed, $\tilde{\eta}_t(F_{n_k}, \gamma',\cdot)$ and $\tilde{\eta}_t(F, \gamma',\cdot)$ are by definition harmonic extensions of functions whose boundary values differ by at most the right hand side. Since $\sup_{x\in \R}|F(x)-F_{n_k}(x)| \to 0$ by assumption, we may conclude that, for any $T>0$, almost surely as $k\to\infty$, 
\begin{equation} \label{eqn::weakconvergence2}
\sup_{t\in [0, T]}\left|\tilde{\eta}_t(F_{n_k}, \gamma^{(n_k)},z)- \tilde{\eta}_t(F, \gamma^{(n_k)},z)\right|\to 0 .
\end{equation} 
Combining Equations (\ref{eqn::weakconvergence1}) and (\ref{eqn::weakconvergence2}), we obtain the conclusion.
\end{proof}

\begin{proof}
[Proof of Proposition \ref{propn::weaklimit}, Item (3)]
Fix $z\in \HH$. Since $\gamma^{(n_k)}$ is coupled as a level line of $h+F_{n_k}$ we know by Lemma \ref{lem::coupling_iff_martingale} that $\left(\tilde{\eta}_t(F_{n_k}, \gamma^{(n_k)},z)\right)_{t\geq 0}$ is a Brownian motion for each $k$.  Therefore, by the weak convergence in Lemma \ref{lemma::etaconvergence}, we have that if $\gamma$ is the limiting law of the $\gamma^{(n_k)}$'s, the process $\tilde{\eta}_t(F, \gamma,z)$ must also have the law of Brownian motion. Applying Lemma \ref{lem::coupling_iff_martingale} again proves the proposition.
\end{proof}

\begin{proof}
[Proof of Lemma \ref{lem::tildeeta_cvg_gamma}]
Fix $z\in \HH$. We will show that the laws of $(\tilde{\eta}_t(F, \gamma^{(n_k)},z))_{t\geq 0}$ converge weakly in $k$ to the law of $(\tilde{\eta}_t(F, \gamma,z))_{t\geq 0}$. To do this, we begin by showing that this family of laws is tight in the space of real valued functions on $[0,\infty)$ with respect to the topology of uniform convergence on compact subsets. This allows us to extract a further subsequence along which the $\tilde{\eta}_t(F, \gamma^{(n_k)},z)$'s converge. We then argue that the limit of this subsequence must be equal to that of $\tilde{\eta}_t(F, \gamma,z)$, so in fact our whole original subsequence converged, and the limit is $\tilde{\eta}_t(F, \gamma,z)$.
Note that the proof of this lemma would be trivial if $\tilde{\eta}_t(F, \cdot, z)$ was a continuous function on the set of curves, however, this is not quite the case. It is essentially a continuous function when restricted to a set in which the $\gamma^{(n_k)}$'s lie with high probability. 

By the proof of \cite[Theorem 1.5]{ksrc}, we know that for every $M>0$ we can find a subset $E$ of the space of continuous curves in $\HH$ such that
\begin{equation} \label{tight} \inf_{k} \PP(\gamma^{(n_k)}\in E) \geq 1-\frac{1}{M} \end{equation}
when the $(\gamma^{(n_k)})$ are parameterised by half plane capacity, and 
\begin{itemize}
\item $E$ is relatively compact with respect to the topology of uniform convergence on compacts,
\item curves in $E$ correspond to Loewner chains with continuous driving functions parameterised by half plane capacity, and
\item if a sequence of curves in $E$ converges with respect to uniform convergence on compacts, then their driving functions also converge uniformly on compacts along a further subsequence, and the limits agree.
\end{itemize}
{\color{blue} For the construction of such an $E$, see Section 3.5 of \cite{ksrc}, in particular the definition (60) and the discussion in the closing paragraphs. See also the opening paragraph of Section 3.6.}

We argue that the image of $E$ under $\tilde{\eta}_t(F, \cdot, z)$ is a relatively compact subset of the space of continuous real-valued functions on $[0,\infty)$ with respect to the topology of uniform convergence on compacts. Thus by (\ref{tight}) the laws of the $(\tilde{\eta}_t(F, \gamma^{(n_k)},z))_{t\geq 0}$ are tight in this topology. 
It is sufficient to verify the following claim: if $\gamma_n'\to \gamma'$ is any convergent sequence of curves in $E$, whose driving functions also converge uniformly {\color{blue} on compacts}, then for any $T>0$, as $n\to\infty$,
\begin{equation}\label{eqn::tildeeta_cvg_nicegamma}
\sup_{t\in [0,T]}\left| \tilde{\eta}_t(F, \gamma_n',z) - \tilde{\eta}_t(F, \gamma',z)\right| \to 0.
\end{equation}
Relative compactness then follows because the choice of $E$ means that any sequence of curves in $E$ has a convergent subsequence along which the driving functions also converge. 

We will prove the above claim now. We let $K_t$ (resp. $K_t^n$) be the hull generated by $\gamma'$ (resp. $\gamma_n'$) and $W_t, g_t$ (resp. $W_t^n, g_t^n$) be the corresponding driving functions {\color{blue} and functions $\HH\setminus K_t$ (resp. $\HH\setminus K_t^n$) to $\HH$, normalised at $\infty$}. We define $f_t=g_t-W_t$ and $f_t^n=g_t^n-W_t^n$ as usual, and consider these to be extended to the boundary, also writing $f_t(0^+)$ for $V_t^R(0^+)-W_t$. Write 
\[C_t=C_t(\gamma', z),\quad C_t^n=C_t(\gamma_n', z);\]
\[\tau(t):= \inf\{s\geq 0: C_s=t\}, \quad \tau^n(t):= \inf\{s\geq 0: C_s^n=t\}. \]

First, we will show that for any $T>0$ before the first time that $\gamma'$ swallows $z$,  as $n\to\infty$,
\begin{equation}
\label{eqn::tildeeta_cvg_nicegamma1}
\sup_{t\in[0,T]}|C_t-C_t^n| \to 0.
\end{equation}

We have the following observations.
\begin{itemize}
\item By Lemma \ref{lem::cr_evolution} we have
\[C_t-C_0=\int_0^t \frac{-4\Im(f_s(z))^2}{|f_s(z)|^4} ds;\quad C^n_t-C_0=\int_0^t \frac{-4\Im(f^n_s(z))^2}{|f^n_s(z)|^4} ds.\]
\item $W_t^n\to W_t$ uniformly on $[0, T]$.
\item $g_t^n \to g_t$ uniformly on $\{(t,z)\in [0,T]\times \overline{\HH}: d(z,K_t)>\delta\}$ for any $\delta>0$. (See for instance \cite[Lemmas A.3 and A.4]{ksrc}) 
\end{itemize}
Combining these three facts, we obtain Equation (\ref{eqn::tildeeta_cvg_nicegamma1}).
\medbreak
Second, we show that, for any $T>0$ before $\gamma'$ swallows $z$, as $n\to\infty$, 
\begin{equation}\label{eqn::tildeeta_cvg_nicegamma2}
\sup_{t\in [0,T]}\left|\eta_{\tau^n(t)}(F, \gamma',z)-\eta_{\tau(t)}(F, \gamma',z) \right|\to 0. 
\end{equation}
By Equation (\ref{eqn::tildeeta_cvg_nicegamma1}), we have that $[0,\tau^n(T)\vee \tau(T)]\subset [0,\tau(S)]$ for $n$ large enough, where $S>T$, and $\tau(S)$ is a time before $z$ is swallowed by $\gamma'$. By (\ref{eqn::tildeeta_cvg_nicegamma1}) again, we therefore have that, as $n\to\infty$ \[c_n:=\sup_{t\in [0,T]}|C_{\tau^n(t)}-t|\le \sup_{t\in [0,\tau^n(T)\vee \tau(T)]}|C_t - C_t^n |\to 0.\]
Since
\[\sup_{t\in [0,T]}\left|\eta_{\tau^n(t)}(F, \gamma',z)-\eta_{\tau(t)}(F, \gamma',z) \right|
\le \sup_{s,t\in [0,S], |s-t|\leq c_n}\left| \tilde{\eta}_t(F, \gamma',z) - \tilde{\eta}_s(F, \gamma',z)\right|,\]
and $\tilde{\eta}_t(F, \gamma',z)$ is uniformly continuous on $[0,S]$, we see that it must converge to $0$.

\medbreak
Third, we show that, for any $T>0$ before $\gamma'$ swallows $z$, as $n\to\infty$, 
\begin{equation}\label{eqn::tildeeta_cvg_nicegamma3}
\sup_{t\in [0,T]} \left|\eta_{\tau^n(t)}(F, \gamma_n',z)-\eta_{\tau^n(t)}(F, \gamma',z) \right|\to 0. 
\end{equation}
We need only show that, on any time interval $[0,S]$ such that $S$ is strictly less than the time $\gamma'$ swallows $z$,  the quantity $\left|\eta_t(F, \gamma_n',z)-\eta_t(F, \gamma',z)\right|$ converges uniformly to $0$. We have the following observations.
\begin{itemize}
\item By Definition \ref{defn::etatilde}, we know that $\eta_t(F, \gamma', \cdot)$ (resp. $\eta_t(F, \gamma_n', \cdot)$) is the harmonic function with boundary values equal $F$ on $\R\setminus K_t$ (resp. on $\R\setminus K^n_t$), $-\lambda$ on the left side of $K_t$ (resp. $K^n_t$), and $\lambda$ on the right side of $K_t$ (resp. $K^n_t$).
\item $W_t^n\to W_t$ uniformly on $[0, S]$.
\item $g_t^n \to g_t$ uniformly on $\{(t,z)\in [0,S]\times \overline{\HH}: d(z,K_t)>\delta\}$ for any $\delta>0$. Same reason as above.
\end{itemize}
Combining these three facts, we have that the quantity $\left|\eta_t(F, \gamma_n',z)-\eta_t(F, \gamma',z)\right|$ converges uniformly to $0$ on $t\in [0,S]$, implying Equation (\ref{eqn::tildeeta_cvg_nicegamma3}).
\medbreak
Combining Equations (\ref{eqn::tildeeta_cvg_nicegamma1}), (\ref{eqn::tildeeta_cvg_nicegamma2}) and (\ref{eqn::tildeeta_cvg_nicegamma3}), we obtain Equation (\ref{eqn::tildeeta_cvg_nicegamma}) by noting that 
\[\sup_{t\in [0,T]}\left| \eta_{\tau^n(t)}(F, \gamma_n',z)-\eta_{\tau(t)}(F, \gamma',z) \right| \leq \sup_{t\in [0,T]} \left|\eta_{\tau^n(t)}(F, \gamma_n',z)-\eta_{\tau^n(t)}(F, \gamma',z) \right| + \sup_{t\in [0,T]}\left|\eta_{\tau^n(t)}(F, \gamma',z)-\eta_{\tau(t)}(F, \gamma',z) \right|.\]
\medbreak
Finally, we show that if $(\gamma^{(n_k)})_{k\in \N}$ converges weakly, and there exists a further subsequence along which $\tilde{\eta}_t(F, \gamma^{(n_k)},z)$ converges, then the limit must be $\tilde{\eta}_t(F, \gamma,z)$.
To do this, for any $M\in \N$ take $E$ relatively compact such that (\ref{tight}) holds, and note that by the above claim we have that
\[A_E:=\left\{(\gamma', \tilde{\eta}(F, \gamma',z)): \gamma' \in E\right\}\] is relatively compact in $C([0,\infty);\C)\times C([0,\infty);\R)$ , and its closure is equal to 
\[\left\{(\gamma', \tilde{\eta}(F, \gamma',z)): \gamma' \in \overline{E}\right\}.\]
This means that the joint laws of $(\gamma^{(n_k)}, \tilde{\eta}(F,\gamma^{(n_k)},z))$ are also tight, and thus we can extract an even further subsequence along which we have joint convergence. If $\PP^*$ is the law of this joint limit then, 
\[ \PP^*\left(\overline{A_E}\right)\geq \inf_k \PP\left( \gamma^{(n_k)} \in \overline{E} \right) \geq 1- \frac{1}{M} \] and so we see that the 
probability of our two marginal laws agreeing in the sense we want must be greater than $1-\frac{1}{M}$. Since this holds for every $M$, agreement must hold almost surely, and as these marginal laws are equal to the limiting laws of the individually convergent sequences, the result follows. 
 
\end{proof}


